An Online Hierarchical Algorithm for Extreme Clustering

Many modern clustering methods scale well to a large number of data items, N, but not to a large number of clusters, K. This paper introduces PERCH, a new non-greedy algorithm for online hierarchical clustering that scales to both massive N and K--a problem setting we term extreme clustering. Our algorithm efficiently routes new data points to the leaves of an incrementally-built tree. Motivated by the desire for both accuracy and speed, our approach performs tree rotations for the sake of enhancing subtree purity and encouraging balancedness. We prove that, under a natural separability assumption, our non-greedy algorithm will produce trees with perfect dendrogram purity regardless of online data arrival order. Our experiments demonstrate that PERCH constructs more accurate trees than other tree-building clustering algorithms and scales well with both N and K, achieving a higher quality clustering than the strongest flat clustering competitor in nearly half the time.

==> alg_multisearch.tex <==
\begin{algorithm}[h]
   \caption{MULTISEARCH}
   \label{alg:multisearch}
\begin{algorithmic}
   \STATE {\bfseries Input:} data point $x_i$, cluster tree $T$
   \STATE $b = T.$\texttt{ROOT}$())$
   \IF{$b.$\texttt{IS\_LEAF}$()$}
   \STATE {\bfseries Output:} $b$
   \ENDIF
   \STATE $h = $ \texttt{NEW\_MINHEAP}$()$
   \STATE $d = $ \texttt{MIN\_DIST}$(x_i, b)$
   \STATE $h.$\texttt{PUSH}$(d,b)$
   \WHILE{$h.$\texttt{NOT\_EMPTY}$()$}
   \STATE $(\_, t) = h.$\texttt{POP}$()$
   \IF{$t.$\texttt{CHILDREN}$()$}
   \FOR{$c$ in $t.$\texttt{CHILDREN}$()$}
   \STATE $d = $ \texttt{MIN\_DIST}$(x_i, c)$
   \STATE $h.$\texttt{PUSH}$(d,c)$
   \ENDFOR
   \ELSE
   \STATE {\bfseries Output:} $c$
   \ENDIF
   \ENDWHILE
\end{algorithmic}
\end{algorithm}


==> robustness_f1.tex <==
\begin{tabular}{|c| c c |}
\hline
\bf       & Round.  & Sort. \\
\hline
Ours      & 44.77   &  35.28   \\
o-MB-KM   & 41.09   &  19.40   \\
SKM++     & 43.33   &  46.67   \\
\hline
\end{tabular}
\caption{Pairwise F1 on adversarial input orders for ALOI.}
\label{tab:robust-f1}

